A temporally adaptive hybridized discontinuous Galerkin method for time-dependent compressible flows

The potential of the hybridized discontinuous Galerkin (HDG) method has been recognized for the computation of stationary flows. Extending the method to time-dependent problems can, e.g., be done by backward difference formulae (BDF) or diagonally implicit Runge-Kutta (DIRK) methods. In this work, we investigate the use of embedded DIRK methods in an HDG solver, including the use of adaptive time-step control. Numerical results demonstrate the performance of the method for both linear and nonlinear (systems of) time-dependent convection-diffusion equations.

==> adjoint_time.tex <==
As usual in the use of adjoint methods, the desire is to taylor-suit an algorithm particularly to maximize the quality of a given \emph{target functional}. In this publication, we consider the target functional at final time $T$, 
%
\begin{align}
 \label{eq:target_fctl}
  J(w) := \int_{\Omega} \xi(w(\cdot, T)) \ dx.
\end{align}
%
It is well-known that the adjoint equation associated with \eqref{eq:conv_diff} and the target functional \eqref{eq:target_fctl} is given as 
%
\begin{alignat}{2}
 \label{eq:adj_conv_diff}
 -z_t - \left( \left(\partial_w f(w)\right)^T - \left(\partial_w f_v(w)\right)^T \right) \nabla z - \nabla \cdot \left( \left( \partial_{\nabla w} f_v(w, \nabla w) \right)^T \nabla z \right) &= 0 &\quad& \forall (x, t) \in \Omega \times (0, T) \\
 w(x, T) &= \xi'(w(\cdot, T)) &\quad& \forall x \in \Omega,
\end{alignat}
%
again subject to suitable boundary values, see, e.g., \cite{Jameson1988, RHa}. 
Given the adjoint has been computed, the error in the target functional can to first order be expressed as a scalar product of $z$ and the residual of the function $w_h$ approximating $w$, i.e., 
%
\begin{align}
  e_h := J(w) - J(w_h) \approx (z, R(w_h))_{\Omega \times (0, T)}, 
\end{align}
%
where the scalar product involves integration over both time and space. 


In \cite{SM12}, we have shown that the hybridized method \eqref{eq:hybrid} is \emph{adjoint consistent} in the stationary case. This means that the algorithm, defined by finding the vector $\zz_h := (\tau_h^z, \varphi_h^z, \mu_h^z) \in H_h \times V_h \times M_h$, such that
%
\begin{alignat*}{2}
 N'(\ww_h)(\xx_h, \zz_h) &= J'(\ww_h)(\xx_h) &\quad& \forall \xx_h \in \XX_h,
\end{alignat*}
%
is a \emph{consistent} discretization of the stationary version of \eqref{eq:adj_conv_diff}. More precisely, 
%
\begin{alignat*}{2}
 N'(\ww)(\xx_h, \zz) = J'(\ww)(\xx_h) &\quad& \forall \xx_h \in \XX_h
\end{alignat*}
%
holds for $\zz := (-\nabla z, z, z_{|\Gamma_0})$. 

This result makes it particularly simple to approximate \eqref{eq:adj_conv_diff} in our setting: A consistent discretization is given as 
%
\begin{alignat}{2}
        -T((z_h)_t, \varphi_h) + N'(w_h)(\xx_h, \zz_h) &= J'(\ww_h)(\xx_h) &\quad& \forall \xx_h \in \XX_h.
\end{alignat}
%
Furthermore, extending the error-estimation methodology from the stationary case scenario to the unsteady scenario CITEMICHAEL, we can consider the the error estimator
%
\begin{align}
        e_h \approx ....
\end{align}
%
%\begin{itemize}
% \item Combine adjoint consistency in the stationary case with time-dependency, using $T$.
% \item Derive an error estimator, both in the continuous and discrete version. 
%\end{itemize}

